Similarity-based Neighbor Selection for Graph LLMs

Text-attributed graphs (TAGs) present unique challenges for direct processing by Language Learning Models (LLMs), yet their extensive commonsense knowledge and robust reasoning capabilities offer great promise for node classification in TAGs. Prior research in this field has grappled with issues such as over-squashing, heterophily, and ineffective graph information integration, further compounded by inconsistencies in dataset partitioning and underutilization of advanced LLMs. To address these challenges, we introduce Similarity-based Neighbor Selection (SNS). Using SimCSE and advanced neighbor selection techniques, SNS effectively improves the quality of selected neighbors, thereby improving graph representation and alleviating issues like over-squashing and heterophily. Besides, as an inductive and training-free approach, SNS demonstrates superior generalization and scalability over traditional GNN methods. Our comprehensive experiments, adhering to standard dataset partitioning practices, demonstrate that SNS, through simple prompt interactions with LLMs, consistently outperforms vanilla GNNs and achieves state-of-the-art results on datasets like PubMed in node classification, showcasing LLMs' potential in graph structure understanding. Our research further underscores the significance of graph structure integration in LLM applications and identifies key factors for their success in node classification. Code is available at https://github.com/ruili33/SNS.

==> future.tex <==
\section*{Future Works}
In this study, our primary focus has been on the selection of top-k neighbors for determining the most relevant connections. However, there are various probabilistic sampling methods available, such as top-k sampling \cite{fan2018hierarchical,holtzman2018learning,radford2019language} and nucleus sampling \cite{holtzman2019curious}, that could further refine this process. Integrating these techniques into neighbor selection might enhance the diversity of the chosen neighbors while maintaining their quality. Our central contributions in this work emphasize the impressive capabilities of LLMs in handling graph data and the critical role of selecting suitable neighbors. Exploring these additional probabilistic methods presents a promising avenue for future research.
